GroundCount: Grounding Vision-Language Models with Object Detection for Mitigating Counting Hallucinations

Vision Language Models (VLMs) exhibit persistent hallucinations in counting tasks, with accuracy substantially lower than other visual reasoning tasks (excluding sentiment). This phenomenon persists even in state-of-the-art reasoning-capable VLMs. Conversely, CNN-based object detection models (ODMs) such as YOLO excel at spatial localization and instance counting with minimal computational overhead. We propose GroundCount, a framework that augments VLMs with explicit spatial grounding from ODMs to mitigate counting hallucinations. In the best case, our prompt-based augmentation strategy achieves 81.3% counting accuracy on the best-performing model (Ovis2.5-2B) - a 6.6pp improvement - while reducing inference time by 22% through elimination of hallucination-driven reasoning loops for stronger models. We conduct comprehensive ablation studies demonstrating that positional encoding is a critical component, being beneficial for stronger models but detrimental for weaker ones. Confidence scores, by contrast, introduce noise for most architectures and their removal improves performance in four of five evaluated models. We further evaluate feature-level fusion architectures, finding that explicit symbolic grounding via structured prompts outperforms implicit feature fusion despite sophisticated cross-attention mechanisms. Our approach yields consistent improvements across four of five evaluated VLM architectures (6.2--7.5pp), with one architecture exhibiting degraded performance due to incompatibility between its iterative reflection mechanisms and structured prompts. These results suggest that counting failures stem from fundamental spatial-semantic integration limitations rather than architecture-specific deficiencies, while highlighting the importance of architectural compatibility in augmentation strategies.

==> algorithms/fusionblock.tex <==
\begin{algorithm}[ht]
\caption{FusionBlock: Cross-Modal Feature Integration}
\label{alg:fusionblock}
\begin{algorithmic}[1]
\REQUIRE ViT tokens $\mathbf{H} \in \mathbb{R}^{B \times T \times C_v}$, DETR features $\mathbf{D} \in \mathbb{R}^{B \times C_d}$
\ENSURE Fused representations $\mathbf{F} \in \mathbb{R}^{B \times T \times C_o}$
\STATE $\mathbf{H}_n \gets \text{LayerNorm}(\mathbf{H})$
\STATE $\mathbf{D}_n \gets \text{LayerNorm}(\mathbf{D})$
\STATE $\mathbf{H}_{\text{cross}} \gets \text{CrossAttn}(\mathbf{H}_n, \mathbf{D}_n)$
\STATE $\mathbf{H}' \gets \text{LayerNorm}(\mathbf{H}_n + \mathbf{H}_{\text{cross}})$
\STATE $[\gamma, \beta] \gets \text{Split}(\text{MLP}_{\text{FiLM}}(\mathbf{D}_n))$
\STATE $\mathbf{H}_{\text{mod}} \gets \mathbf{H}' \odot (1 + \gamma) + \beta$
\STATE $\mathbf{D}_{\text{exp}} \gets \text{Expand}(\mathbf{D}_n, T)$ \Comment{Replicate to match spatial dims}
\STATE $\mathbf{C} \gets \text{LayerNorm}([\mathbf{H}_{\text{mod}}, \mathbf{D}_{\text{exp}}])$ \Comment{Concatenate}
\STATE $\mathbf{A} \gets \text{MLP}_A(\mathbf{C})$
\STATE $\mathbf{g}_v \gets \tanh(W_v \cdot \mathbf{H}_{\text{mod}})$
\STATE $\mathbf{g}_d \gets \tanh(W_d \cdot \mathbf{D}_n)$
\STATE $\mathbf{B} \gets \text{MLP}_B([\mathbf{H}_{\text{mod}} \odot \mathbf{g}_v, \mathbf{D}_{\text{exp}} \odot \mathbf{g}_d])$
\STATE $[\alpha_0, \alpha_1] \gets \text{Softmax}(\mathbf{w})$ \Comment{Learnable branch weights}
\STATE $\mathbf{X} \gets \alpha_0 \mathbf{A} + \alpha_1 \mathbf{B}$
\STATE $\mathbf{X} \gets \text{LayerNorm}(\mathbf{X})$
\STATE $\mathbf{X} \gets \mathbf{X} + \text{MLP}_{\text{bottleneck}}(\mathbf{X})$
\STATE $\mathbf{X} \gets \mathbf{X} + \lambda \cdot \text{MLP}_{\text{inject}}(\mathbf{D}_{\text{exp}})$ \Comment{$\lambda$ is learnable}
\STATE $\mathbf{X} \gets \text{DropPath}(\mathbf{X})$
\STATE $\mathbf{R} \gets W_r \cdot \mathbf{H}$ \Comment{Project ViT residual if needed}
\STATE $\mathbf{G} \gets \sigma(W_g \cdot \mathbf{D}_n)$ \Comment{DETR-conditioned gate}
\STATE $\mathbf{F} \gets \text{LayerNorm}(\mathbf{X} + \mathbf{G} \odot \mathbf{R})$
\RETURN $\mathbf{F}$
\end{algorithmic}
\end{algorithm}

==> figures/baseline_results.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth, trim={0 7 0 0}, clip]{images/baseline_results.pdf}
    \caption{PhD dataset accuracy by question categories.}
    \label{fig:baseline}
\end{figure*}


==> figures/cover_image.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\columnwidth, trim={71 275 1075 62}, clip]{images/cover_image.pdf}
    \vspace{-0.8cm}
    \caption{CountFormer gives accurate count and tells the locations well.}
    \label{fig:cover_image}
\end{figure}


==> figures/training_pipeline.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth, trim={5 485 325 20}, clip]{images/training_pipeline.pdf}
    \caption{Overview of our training pipeline for vision-language model development. The pipeline consists of multiple stages including data preprocessing, multi-modal alignment, and fine-tuning phases.}
    \label{fig:training_pipeline}
\end{figure*}

==> tables/papers_summary.tex <==
\renewcommand{\arraystretch}{1.55}
\setlength{\tabcolsep}{6pt}
\small

\onecolumn
\begin{longtable}{m{5.6cm} m{4.2cm} m{2.7cm} >{\centering\arraybackslash}m{0.7cm}}
\caption{
\textbf{Overview of hallucination mediation works and their evaluated datasets, VLMs, and whether their methodologies involve model training.}
To facilitate understanding in the SOTA, we list all recent works published in top venues (ICML'25, CVPR'25, NAACL'25, ICLR'25, AAAI'25, NeurIPS'24), their common baseline methods, and their experimental setups. 
The conferences are sequential from most recent to earliest; works in each conference are sequential in alphabetical order. 
In \textbf{Train} column, (\tick) means the method involves training or finetuning, and (\cross) means not; 
(\protect\yellowcircle) means the work proposes both a train-free method and a training method. Among the 40 listed works, 29 are decoding-level, requiring no training. 
We did not include works specifically targeting video understanding. However, a few works (eg. FarSight) can also be applied to video MLLMs. 
\label{tab:work_dataset}
} \\
\toprule
\textbf{Works in Hallucination Optimization} & \textbf{Benchmark/Dataset} & \textbf{VLM} & \textbf{Train} \\
\midrule
\endfirsthead

\toprule
\textbf{Works in Hallucination Optimization} & \textbf{Benchmark/Dataset} & \textbf{VLM} & \textbf{Train} \\
\midrule
\endhead

\bottomrule
\endfoot

\noalign{\vskip 1ex}
\multicolumn{4}{c}{\rule{0.4\textwidth}{0.4pt} \hspace{0.5em} \textit{ICML'25} \hspace{0.5em} \rule{0.4\textwidth}{0.4pt}} \\
\noalign{\vskip 1ex}

\textsc{MARINE} (Mitigating hallucinAtion via classifieR-Free guIdaNcE) \cite{zhao2025mitigating} & POPE, CHAIR & LLaVA-v1.5, LLaVA-v1, InstructBLIP, MiniGPT-2, mPLUG-Owl2, LLaMA-Adapter-v2 & \cross \\
\textsc{MemVR} (Selective and Contrastive Decoding) \cite{zou2025memvr} & POPE, CHAIR, VizQiz-VQA, MME, MMBench, MM-Vet, LLaVA-Bench, HallusionBench & LLaVA-v1.5, Qwen-VL & \cross \\
\textsc{RBD} (Re-Balancing Contrastive Decoding) \cite{zhao2025mitigating} & POPE (MSCOCO), MME, MMBench, VQA-v2, GQA, VizWiz, ScienceQA-IMG, TextVQA & LLaVA-v1.5, InstructBLIP, MiniGPT-4 & \cross \\
\textsc{SECOND} (Selective and Contrastive Decoding) \cite{park2025second} & POPE, MMBench, VQA-v2, MMStar & LLaVA-NEXT, LLaVA-OneVision, Yi-VL & \cross \\
\textsc{VISTA} (Visual Information Steering with Token-logit Augmentation) \cite{li2025the} & POPE (MSCOCO), CHAIR & LLaVA-v1.5, InstructBLIP, MiniGPT-4, Shakira & \cross \\

\noalign{\vskip 1ex}
\multicolumn{4}{c}{\rule{0.4\textwidth}{0.4pt} \hspace{0.5em} \textit{CVPR'25} \hspace{0.5em} \rule{0.4\textwidth}{0.4pt}} \\
\noalign{\vskip 1ex}

% \textsc{AGLA} \cite{Leng_2024_CVPR} & POPE, ROPE, MME, CHAIR, LLaVA-Wild & LLaVA-v1.5, InstructBLIP, Qwen-VL, MiniCPM-V & \cross \\
\textsc{Antidote} \cite{Wu_2025_CVPR} & POPE, CHAIR, CP-Bench, SHR, MMBench, MMVet, Science-QA, LLaVA-Wild & LLaVA-v1.5, LLaVA-NeXT, InstructBLIP, MiniGPT-4 & \tick \\
\textsc{Devils} \cite{jiang2025devils} & CHAIR & LLaVA-v1.5, Shikra, MiniGPT-4 & \cross \\
\textsc{FarSight} \cite{tang2025seeing} & POPE, CHAIR, MMBench, MMVet, LLaVA-Wild, VizWiz, SQA & LLaVA-v1.5, InstructBLIP, VILA & \cross \\
\textsc{ICT} \cite{chen2025ict} & POPE, MME & LLaVA-v1.5, Qwen-VL & \cross \\
\textsc{Nullu} \cite{yang2025nullu} & POPE, CHAIR, MME, LLaVA-Bench & LLaVA-v1.5, MiniGPT-4, mPLUG-Owl2 & \cross \\
\textsc{Octopus} \cite{Wu_2025_CVPR} & CHAIR, Hal, Cog, Cover, GPT-4, AMBER, Object-HalBench, MMHalBench & LLaVA-v1.5, InstructBLIP & \cross \\
\textsc{OPA-DPO} \cite{Wu_2025_CVPR} & POPE (adversarial), CHAIR, AMBER, MMHalBench, Object HalBench,  & LLaVA-v1.5 & \tick \\
\textsc{VAF} (Visual  Amplification  Fusion) \cite{yin2025clearsight} & POPE, MME, NoCaps & LLaVA-v1.5, Qwen-VL & \cross \\
\textsc{VASparse} \cite{zhuang2025vasparse} & POPE (MSCOCO), CHAIR, MME, GPT-4 & LLaVA-v1.5, MiniGPT-4, mPLUG-Owl2 & \cross \\

\noalign{\vskip 1ex}
\multicolumn{4}{c}{\rule{0.4\textwidth}{0.4pt} \hspace{0.5em} \textit{NAACL'25} \hspace{0.5em} \rule{0.4\textwidth}{0.4pt}} \\
\noalign{\vskip 1ex}

\textsc{BBVPE} (Black-Box Visual Prompt Engineering) \cite{woo-etal-2025-black} & POPE, CHAIR, GPT-4o & LLaVA-v1.5, InstructBLIP & \cross \\
\textsc{ContextLens} \cite{phukan-etal-2025-beyond} & HQH, TextVQA-X, VizWiz-G, mAP & Qwen2-VL-7B, internlm-xcomposer2-vl-7b & \cross \\
\textsc{iTaD} (image Token
attention-guided Decoding) \cite{xu-etal-2025-mitigating} & POPE, CHAIR, GPT-4V & LLaVA-v1.5, InstructBLIP, MiniGPT-4, mPLUG-Owl2 & \cross \\
\textsc{SumGD} (Summary-Guided Decoding) \cite{min-etal-2025-mitigating} & CHAIR, SHR & LLaVA-v1.5, InstructBLIP & \cross \\

\noalign{\vskip 1ex}
\multicolumn{4}{c}{\rule{0.4\textwidth}{0.4pt} \hspace{0.5em} \textit{ICLR'25} \hspace{0.5em} \rule{0.4\textwidth}{0.4pt}} \\
\noalign{\vskip 1ex}

\textsc{CausalMM} (structural Causal modeling to MLLMs) \cite{zhou2025mitigating} & POPE, MME, VLind-Bench & LLaVa-v1.5, Qwen-VL2 & \cross \\
\textsc{DAMO} (Decoding by Accumulating Activations MOmentum) \cite{wang2025damo} & POPE (MSCOCO, A-OKVQA), MME, LLaVa-Bench & LLaVa-v1.5, INF-MLLM1, mPLUG-Owl2 & \cross \\
\textsc{DeCo} (Dynamic Correction decoding) \cite{zhang2025selfcorrecting} & POPE (MSCOCO), CHAIR, MME, GPT-4o assisted evaluation & LLaVA-v1.5, MiniGPT-4, Instruct-BLIP, Qwen-VL & \cross \\
\textsc{DeGF} (self-correcting Decoding with Generative Feedback) \cite{zhang2025selfcorrecting} & POPE, CHAIR, MME-Hallucination, MMBench, MMVP, LLaVA-Bench & LLaVA-v1.5, MiniGPT-4 & \cross \\
\textsc{DPA} (Data-augmented Phrase-level Alignment) \cite{sarkar2025mitigating} & CHAIR, MME-Hall, AMBER, MMHal-Bench, HallusionBench, VQA-v2, MM-Vet, TextVQA, MME, LLaVA-Bench & LLaVA-v1.5, VILA-v1.5 & \tick \\
\textsc{ED} (Ensemble Decoding) \cite{cho2025do} & POPE, CHAIR, MME, LLaVA-Bench & LLaVA-v1.5 & \cross \\
Modular Attribution and Intervention \cite{yang2025mitigating} & CHAIR, Nocaps, MM-Vet & LLaVA-v1.5, InstructBLIP, Qwen-VL & \yellowcircle\\
\textsc{PerturboLLaVA} \cite{chen2025perturbollava} & CHAIR, HalFscore & LLaVa-v1.5 & \tick \\
\textsc{SID} (Self-Introspective Decoding) \cite{huo2025selfintrospective} & POPE, CHAIR, GPT-4 assisted benchmark, MME, MMBench, GPT4-V assisted evaluation, MathVista, MMVet, LLaVa-Bench, MMMU, LLaVA-Bench-in-the-Wild & LLaVa-v1.5, InstructBLIP, LLaVa-NeXT & \cross \\
\textsc{TAME} (Dynamic Token Propagation Mechanism) \cite{ghosh2025visual} & POPE, CHAIR, HalluBench & LLaVA-v1.5, MiniGPT-4, InstructBLIP, Shikra & \cross \\
\textsc{VDGD} (Visual Description Grounded Decoding) \cite{ghosh2025visual} & AMBER (visual recognition), SynthDoG (OCR), MMMU (expert-level reasoning), MathVista, MATH-Vision (mathematical reasoning), MMC (chart understanding), MME, HallusionBench & LLaVA-v1.5, LLaVA-NeXT, LLaVA-v1, mPLUG-Owl2, InternLM-X, CogVLM & \cross \\

\noalign{\vskip 1ex}
\multicolumn{4}{c}{\rule{0.4\textwidth}{0.4pt} \hspace{0.5em} \textit{AAAI'25} \hspace{0.5em} \rule{0.4\textwidth}{0.4pt}} \\
\noalign{\vskip 1ex}

\textsc{AdaVIB} \cite{vib2025baineurips} & POPE, CHAIR, LURE & LLaVA-v1.5, MiniGPT-4 & \tick \\
\textsc{ConVis} \cite{ParkLCC25} & POPE, CHAIR, HallusionBench, MME, LLaVA-Bench & LLaVA-v1.5, mPLUG-Owl2, MiniGPT-4 & \cross \\
\textsc{Holistic Reasoning} \cite{wu2025combating} & POPE, AMBER, WHOOPS!-VQA, WHOOPS!-Gen, VQAv2-IDK & LLaVA-v1.5, MiniGPT-2, Qwen-VL, GPT-4 & \cross \\
\textsc{HSA-DPO} (Hallucination Severity-Aware Direct Preference Optimization) \cite{Xiao_Huang_Gan_He_Li_Yu_Shu_Jiang_Zhu_2025} & POPE, CHAIR, AMBER, ObjectHalBench, MHaluBench, MMHal-Bench, Cover, Cog, Hal & LLaVA-v1.5, InstructBLIP, Qwen-VL-Chat, GPT-4, LRV, LLaVA-RLHF, RLHF-V, Silkie, POVID & \tick \\
\textsc{MoLE} (Mixture of Layer Experts) \cite{liang2025mole} & POPE, CHAIR & LLaVA-v1.5, MiniGPT-4, Shikra & \cross \\


\noalign{\vskip 1ex}
\multicolumn{4}{c}{\rule{0.4\textwidth}{0.4pt} \hspace{0.5em} \textit{NeurIPS'24} \hspace{0.5em} \rule{0.4\textwidth}{0.4pt}} \\
\noalign{\vskip 1ex}

\textsc{CCA} (Concentric Causal Attention) \cite{CCA_NEURIPS2024_a76ed4a8} & POPE & Vicuna-7B + CLIP ViT-L/14 & \tick \\
\textsc{HIO} (Hallucination-Induced Optimization) \cite{HIO_NEURIPS2024_dde04099} & POPE (MSCOCO), CHAIR, MME & LLaVa-v1.5, InstructBLIP, MiniGPT-4 & \tick \\
\textsc{LeHaCE} \cite{zhao2025mitigating} & CHAIR, NoCaps & LLaVA-v1, InstructBLIP, mPLUG-Owl(2), MiniGPT-4, Qwen-VL, Gemini-Pro-Vision pro, LLaMA-Adapter-v2, InternLM-XComposer, Lynx, Otter, VPGTrans & \cross \\
\textsc{ROPE} (Recognition-based Object Probing Evaluation) \cite{chen2024multiobject} & MSCOCO-Panoptic, ADE-20K & LLaVA-NeXT, Yi-VL & \cross \\

\noalign{\vskip 1ex}
\multicolumn{4}{c}{\rule{0.4\textwidth}{0.4pt} \hspace{0.5em} \textit{Earlier Baselines} \hspace{0.5em} \rule{0.4\textwidth}{0.4pt}} \\
\noalign{\vskip 1ex}

\textsc{DoLa} (Decoding by Contrasting Layers) \cite{chuang2024dola} & TruthfulQA, FACTOR & LLaMA & \cross \\
\textsc{ICD} (Instruction Contrastive Decoding) \cite{wang-etal-2024-mitigating} & POPE, MME, LLaVA-Bench & LLaVA-v1.5, InstructBLIP, MiniGPT-4 & \cross \\
\textsc{OPERA} (Over-trust Penalty and a Retrospection-Allocation) \cite{Huang2024OPERA} & POPE, CHAIR, GPT-4(o) assisted evaluation & LLaVA-v1.5, MiniGPT-4, InstructBLIP, Shakira & \cross \\
\textsc{VCD} (Visual Contrastive Decoding) \cite{Leng_2024_CVPR} & POPE, MME, LLaVA-Bench & LLaVA-v1.5, InstructBLIP, Qwen-VL & \cross \\
\end{longtable}

\twocolumn

==> tables/results_pope.tex <==
\newcommand{\resultspopenumrows}{6}
\newcommand{\resultspopefirstcolraisebox}{-4.7}

\begin{table}[p]
\scriptsize
\centering
\captionsetup{font=small}
\caption{Main results on POPE tasks. We evaluate the POPE task accuracy of various MLLMs on the MSCOCO, A-OKVQA, and GQA datasets with LLaVa-v1.5 under different decoding settings. \textbf{Regular} refers to the scenario where direct sampling is applied. \textbf{Vision}, \textbf{Language}, and \textbf{Multimodal} refer to vision-only, language-only, and multimodal collaboration variants of \textsc{CausalMM}. The \textbf{bold} and the \underline{underlined} refer to the highest and second highest metrics under each setting, respectively. Each value is followed by the difference relative to regular setting in the parenthesis.}
\vspace{-2.2mm}
\renewcommand{\arraystretch}{1.0}
\setlength{\tabcolsep}{6pt}
\begin{tabular}{>{\raggedright\arraybackslash}p{1.3cm}llcccc}
\toprule
\textbf{Dataset} & \textbf{Setting} & \textbf{Method} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1 Score} \\
\midrule

\multirow{15}{*}{\raisebox{\resultspopefirstcolraisebox em}{\makebox[0pt][l]{MSCOCO}}}
& \multirow{\resultspopenumrows}{*}{Random} 
    & Regular    & 83.53 (0.00) & 92.12 (0.00) & 73.33 (0.00) & 81.66 (0.00) \\
&   & VCD        & 86.40 (2.87) & 94.68 (2.56) & 77.13 (3.80) & 85.01 (3.35) \\
&   & OPERA      & \textbf{89.20} (5.67) & 92.68 (0.56) & \underline{85.26} (11.9) & \textbf{88.81} (7.15) \\
&   & \textbf{Vision}     & 86.46 (2.93) & \underline{96.27} (4.15) & 75.86 (2.53) & 84.86 (3.20) \\
&   & \textbf{Language}   & \underline{88.00} (4.47) & 95.96 (3.84) & 79.33 (6.00) & 86.86 (5.20) \\
&   & \textbf{Multimodal} & 88.93 (5.40) & \textbf{95.20} (3.08) & \textbf{82.00} (8.67) & \underline{88.10} (6.44) \\
\cmidrule{2-7}
& \multirow{\resultspopenumrows}{*}{Popular} 
    & Regular    & 81.10 (0.00) & 87.89 (0.00) & 72.13 (0.00) & 79.23 (0.00) \\
&   & VCD        & 83.53 (2.43) & 89.29 (1.40) & 76.20 (4.07) & 82.23 (3.00) \\
&   & OPERA      & 86.83 (5.73) & 88.24 (0.35) & \textbf{85.26} (13.1) & 86.62 (7.39) \\
&   & \textbf{Vision}     & 84.56 (3.46) & \underline{91.57} (3.68) & 76.13 (3.00) & 84.14 (3.91) \\
&   & \textbf{Language}   & 87.03 (5.93) & \textbf{91.80} (3.91) & 88.13 (16.0) & \textbf{87.17} (7.94) \\
&   & \textbf{Multimodal} & \textbf{87.13} (6.03) & 86.35 (1.46) & \underline{88.20} (16.0) & \underline{87.26} (8.03) \\
\cmidrule{2-7}
& \multirow{5}{*}{Adversarial}
    & Regular    & 78.63 (0.00) & 82.96 (0.00) & 72.06 (0.00) & 77.13 (0.00) \\
&   & VCD        & 81.10 (2.47) & 84.47 (1.51) & 76.20 (4.14) & 80.12 (2.99) \\
&   & OPERA      & 81.13 (2.50) & 78.74 (4.17) & 85.20 (13.1) & 81.87 (4.74) \\
&   & \textbf{Vision}     & 82.20 (3.57) & 86.64 (3.68) & 76.13 (4.07) & 81.81 (4.74) \\
&   & \textbf{Language}   & 81.73 (3.10) & 86.28 (3.32) & 75.46 (3.40) & 80.81 (3.67) \\
&   & \textbf{Multimodal} & \textbf{83.70} (5.07) & \underline{87.69} (4.73) & \textbf{78.40} (6.34) & \underline{82.75} (5.65) \\
\midrule

\multirow{15}{*}{\raisebox{\resultspopefirstcolraisebox em}{\makebox[0pt][l]{A-OKVQA}}}
& \multirow{\resultspopenumrows}{*}{Random}
    & Regular    & 84.03 (0.00) & 87.67 (0.00) & 79.20 (0.00) & 83.22 (0.00) \\
&   & VCD        & 85.90 (1.87) & 88.27 (0.60) & 82.80 (3.60) & 85.44 (2.22) \\
&   & OPERA      & 88.23 (4.20) & 86.13 (1.54) & \textbf{91.13} (11.9) & \textbf{88.11} (4.89) \\
&   & \textbf{Vision}     & 87.66 (3.63) & \underline{90.24} (2.57) & 84.46 (5.26) & 87.25 (4.03) \\
&   & \textbf{Language}   & 85.96 (1.93) & 89.75 (2.08) & 81.20 (2.00) & 85.86 (2.04) \\
&   & \textbf{Multimodal} & \textbf{88.93} (4.90) & \textbf{91.89} (4.22) & \underline{85.40} (6.20) & \underline{88.52} (5.30) \\
\cmidrule{2-7}
& \multirow{\resultspopenumrows}{*}{Popular}
    & Regular    & 80.23 (0.00) & 81.44 (0.00) & 79.20 (0.00) & 80.82 (0.00) \\
&   & VCD        & 81.96 (1.73) & 81.44 (0.57) & 82.80 (3.60) & 82.11 (2.29) \\
&   & OPERA      & 83.40 (3.17) & 78.92 (2.05) & 91.13 (11.9) & 84.59 (4.57) \\
&   & \textbf{Vision}     & 84.03 (3.80) & 83.74 (2.87) & 84.46 (5.26) & 84.10 (4.08) \\
&   & \textbf{Language}   & \underline{85.96} (5.73) & 89.75 (8.88) & \textbf{81.20} (2.00) & \textbf{85.26} (4.45) \\
&   & \textbf{Multimodal} & \textbf{85.70} (5.47) & \textbf{92.60} (11.17) & \underline{77.60} (1.60) & \underline{84.43} (4.41) \\
\cmidrule{2-7}
& \multirow{5}{*}{Adversarial}
    & Regular    & 74.26 (0.00) & 72.33 (0.00) & 78.60 (0.00) & 75.33 (0.00) \\
&   & VCD        & 76.10 (1.84) & 72.90 (0.57) & 85.06 (6.46) & 77.55 (2.32) \\
&   & OPERA      & 73.90 (-0.36) & 67.77 (-4.56) & \textbf{91.13} (12.53) & \textbf{84.59} (9.26) \\
&   & \textbf{Vision}     & 76.86 (2.60) & 73.43 (1.10) & 80.33 (1.73) & 78.44 (3.11) \\
&   & \textbf{Language}   & 77.43 (3.17) & \underline{74.98} (2.65) & 77.60 (1.60) & 77.08 (1.75) \\
&   & \textbf{Multimodal} & \textbf{77.86} (3.60) & \textbf{74.41} (2.08) & \underline{84.93} (6.33) & \underline{79.32} (3.99) \\
\midrule

\multirow{15}{*}{\raisebox{\resultspopefirstcolraisebox em}{\makebox[0pt][l]{GQA}}}
& \multirow{\resultspopenumrows}{*}{Random}
    & Regular    & 83.60 (0.00) & 87.11 (0.00) & 78.86 (0.00) & 82.78 (0.00) \\
&   & VCD        & 85.86 (2.26) & 88.21 (1.10) & 82.80 (3.94) & 85.41 (2.63) \\
&   & OPERA      & 88.20 (4.60) & 86.13 (1.54) & \textbf{91.13} (12.3) & \textbf{88.51} (5.73) \\
&   & \textbf{Vision}     & 87.40 (3.80) & \underline{90.53} (3.42) & 83.43 (4.67) & 88.06 (4.11) \\
&   & \textbf{Language}   & 86.56 (2.96) & 90.24 (3.13) & 85.06 (6.20) & 85.93 (3.14) \\
&   & \textbf{Multimodal} & \textbf{88.50} (4.90) & \textbf{90.81} (3.70) & \underline{85.66} (6.80) & \underline{88.16} (5.38) \\
\cmidrule{2-7}
& \multirow{\resultspopenumrows}{*}{Popular}
    & Regular    & 77.86 (0.00) & 78.00 (0.00) & 78.86 (0.00) & 78.08 (0.00) \\
&   & VCD        & 79.06 (1.20) & 77.04 (-0.97) & 82.80 (3.94) & 80.60 (2.52) \\
&   & OPERA      & 79.80 (1.94) & 77.43 (-0.57) & 82.80 (3.94) & 82.42 (4.04) \\
&   & \textbf{Vision}     & 79.13 (1.27) & \underline{80.36} (2.36) & 83.40 (4.53) & 81.72 (3.64) \\
&   & \textbf{Language}   & 79.93 (2.07) & 78.70 (0.70) & 83.06 (4.20) & 82.35 (2.27) \\
&   & \textbf{Multimodal} & \textbf{82.36} (4.50) & \textbf{80.36} (2.04) & \underline{85.66} (6.80) & \textbf{82.93} (4.85) \\
\cmidrule{2-7}
& \multirow{5}{*}{Adversarial}
    & Regular    & 75.16 (0.00) & 73.31 (0.00) & 78.00 (0.00) & 76.61 (0.00) \\
&   & VCD        & 76.33 (1.17) & 73.21 (-0.10) & 83.00 (5.00) & 77.55 (0.94) \\
&   & OPERA      & 76.80 (1.64) & 71.36 (-1.95) & \textbf{88.00} (10.0) & \textbf{78.77} (2.17) \\
&   & \textbf{Vision}     & 76.60 (1.44) & 73.43 (0.12) & 82.66 (4.67) & 77.40 (0.79) \\
&   & \textbf{Language}   & 77.40 (2.24) & \underline{74.98} (1.67) & 81.26 (3.13) & 77.70 (1.09) \\
&   & \textbf{Multimodal} & \textbf{79.53} (4.37) & \textbf{76.49} (3.18) & \underline{85.26} (6.13) & \underline{80.64} (3.03) \\
\bottomrule
\end{tabular}
\end{table}

